Computational Paths -- An approach in the $LND_{EQ}-TRS_{2}$ system

We use a labelled deduction system ( LND$_{ED-}$TRS ) based on the concept of computational paths (sequences of rewrites) as equalities between two terms of the same type, which allowed us to carry out in homotopic theory an approach using the concept of computational paths. From this, we show that the computational paths can be used to perform the proofs of the $LND_{EQ}-TRS_{2}$ rewriting system.

==> acronimos.tex <==


% CriaÃ§Ã£o de glossÃ¡rios e lista de abreviaÃ§Ãµes
%\usepackage[smallcaps}{glossaries}
\usepackage{amssymb}

\newacronym{zfc}{ZFC}{Zermelo-Frankel-Choice}
\newacronym{pif}{$\Pi - F$}{dependent function formation}
\newacronym{pii}{$\Pi - I$}{dependent function introduction}
\newacronym{pie}{$\Pi - E$}{dependent function elimination}
\newacronym{pic}{$\Pi - C$}{dependent function computation}
\newacronym{sif}{$\Sigma - F$}{dependent sum formation}
\newacronym{sii}{$\Sigma - I$}{dependent sum introduction}
\newacronym{sie1}{$\Sigma - E_{1}$}{first dependent sum elimination}
\newacronym{sie2}{$\Sigma - E_{2}$}{second dependent sum elimination}
\newacronym{sic}{$\Sigma - C$}{Computação da Soma Dependente}
\newacronym{n0}{$\mathbb N-I_{0}$}{zero introduction}
\newacronym{ns}{$\mathbb N-I_{s}$}{successor induction}
\newacronym{ifi}{$Id^{int} - I$}{identity type introduction}
\newacronym{iff}{$Id^{int} - F$}{identity type formation}
\newacronym{ie}{$Id - E$}{identity type elimination}
\newacronym{ii}{$Id - Eq$}{identity type equality}
\newacronym{ife}{$Id^{ext} - F$}{extensional identity type formation}
\newacronym{iie}{$Id^{ext} - I$}{extensional identity type introduction}
\newacronym{iee}{$Id^{ext} - E$}{extensional identity type elimination}
\newacronym{iei}{$Id^{ext} - Eq$}{extensional identity type equality}
\newacronym{bi}{$\lambda\beta\eta$}{Teoria da Beta-Eta Igualdade}
\newacronym{pf}{$\times - F$}{product formation}
\newacronym{pi}{$\times - I$}{product introduction}
\newacronym{pe1}{$\times - E_{1}$}{first product elimination}
\newacronym{pe2}{$\times - E_{2}$}{second product elimination}
\newacronym{rw}{$LND_{EQ}-TRS$}{Term Rewrite System}
\newacronym{uip}{UIP}{Uniqueness of Identity Proofs}

==> glossaries.tex <==




\newglossaryentry{naive-bayes}
{
  name=\textit{Na{\"i}ve Bayes},
  description={},
  plural=\textit{Na{\"i}ve Bayes}
}

\newglossaryentry{hoeffding-tree}
{
  name=\textit{Hoeffding Tree},
  description={},
  plural=\textit{Hoeffding Trees}
}




\newglossaryentry{data-stream}
{
  name=\textit{Data Stream},
  description={},
  plural=\textit{Data Streams}
}


\newglossaryentry{single-detection-approach}
{
  name=\textit{Single Detection Approach},
  description={},
  plural=\textit{Single Detection Approachs}
}



\newglossaryentry{multiple-detection-approach}
{
  name=\textit{Multiple Detection Approach},
  description={},
  plural=\textit{Multiple Detection Approachs}
}

\newglossaryentry{single-detection}
{
  name=\textit{Single Detection},
  description={},
  plural=\textit{Single Detectors}
}


\newglossaryentry{single-detector}
{
  name=\textit{Single Detector},
  description={},
  plural=\textit{Single Detectors}
}



\newglossaryentry{multiple-classifier-system}
{
  name=\textit{Multiple classifier System},
  description={},
  plural=\textit{Multiple classifier Systems}
}
 

\newglossaryentry{prequential}
{
  name=\textit{Prequential},
  description={},
  plural=\textit{}
}


\newglossaryentry{single-classifier-base}
{
  name=\textit{Single Classifier-base},
  description={},
  plural=\textit{Single classifiers-base}
}

\newglossaryentry{multiple-processing-approach}
{
  name=\textit{Multiple Processing Approach},
  description={},
  plural=\textit{Multiple Processing Approachs}
}

\newglossaryentry{concept-drift}
{
  name=\textit{Concept Drift},
  description={},
  plural=\textit{Concept Drifts}
}


\newglossaryentry{multiple-detector}
{
  name=\textit{Multiples Detector},
  description={},
  plural=\textit{Multiples Detectors}
}

\newglossaryentry{single-detection-algorithm}
{
  name=\textit{Single Detection Algorithm},
  description={},
  plural=\textit{Single Detection Algorithms}
}

\newglossaryentry{ensemble-methods}
{
  name=\textit{Ensemble Methods},
  description={},
  plural=\textit{Ensembles Methods}
}












==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{email} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{email} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.



\end{thebibliography}


